Towards an Accessible, Noninvasive Micronutrient Status Assessment Method: A Comprehensive Review of Existing Techniques

Nutrients are critical to the functioning of the human body and their imbalance can result in detrimental health concerns. The majority of nutritional literature focuses on macronutrients, often ignoring the more critical nuances of micronutrient balance, which require more precise regulation. Currently, micronutrient status is routinely assessed via complex methods that are arduous for both the patient and the clinician. To address the global burden of micronutrient malnutrition, innovations in assessment must be accessible and noninvasive. In support of this task, this article synthesizes useful background information on micronutrients themselves, reviews the state of biofluid and physiological analyses for their assessment, and presents actionable opportunities to push the field forward. By taking a unique, clinical perspective that is absent from technological research on the topic, we find that the state of the art suffers from limited clinical relevance, a lack of overlap between biofluid and physiological approaches, and highly invasive and inaccessible solutions. Future work has the opportunity to maximize the impact of a novel assessment method by incorporating clinical relevance, the holistic nature of micronutrition, and prioritizing accessible and noninvasive systems.

==> Sections/4_remote-assess.tex <==
% \paragraph{Background} 
Since the COVID-19 pandemic, there has been a growing push for assessment methods that don't require a clinician to be physically present \cite{hummell_role_2022, mauldin_performing_2021, shah_evolution_2021}. These remote assessments use telehealth technology to carry out clinical evaluations and NFPEs.
% \subsubsection{Remote NFPE}
Many components of the NFPE remain the same in the remote setting, with an increased reliance on activity tracking devices when assessing a patient's functional status. Observing a patient's living space during a telehealth call is another useful way a way to gain insights into nutritional intake, food availability, and quality of life. The visual inspection of ROIs and the analysis of health data is critical to conducting a remote NFPE. A video call or a collection of photos is especially helpful, as the nutritionist can visually inspect ROIs like they would in-person. It is recommended to start with the oral cavity since it has many early signs of deficiency \cite{hummell_role_2022}. 
Health tracking devices can be useful for a remote exam, providing the practitioner with biometric and physical activity data that can guide a telehealth visit and/or nutritional intervention. Consumer-level scales, bioelectrical impedance analysis (BIA) devices, blood glucose monitors, blood pressure monitors, sleep trackers, and activity trackers are readily available as sources of these data.

Verbal questioning can also be a valuable source of information for remote nutrition assessments, especially for less tech-savvy patients or when photo sharing or video calls are not possible. Researchers recommend asking the patient a series of specific questions to guide them through a virtual head-to-toe examination \cite{mauldin_performing_2021, shah_evolution_2021}.
\citet{chizmar_questionnaire_2022} assessed the correlation between patient responses to verbal questions from a clinician and “physical signs of malnutrition” to validate assessments of nutrition without a physical exam. 
% A study was conducted with 30 patients where their responses to verbal questions were compared to physical exam findings of general malnutrition and indicators thereof (muscle and fat loss, fluid accumulation, and reduced handgrip strength).
A set of four questions about eye and rib appearance, percieved skinniness, and intake changes from swelling were significantly associated with a diagnosis of malnutrition. These and other questions were further associated with other individual factors of malnutrition. As to be expected, this study has few specific implications for micronutrition, but it’s findings are nonetheless useful for the diagnosis of nutrition as a whole.
It should be noted that of these 30 patients, 22 were White and 28 were male. This is critical, as female and non-White patients are disproportionately affected by the burden of malnutrition \cite{pfeiffer_cdcs_2013, kawano_racial_2024}. 

% \subsubsection{Remote Dietary Assessment}
In remote dietary assessment, most new innovations are app-based \cite{mauldin_performing_2021}. These methods can act as intake loggers: users can input their dietary history, and nutritional metrics can be calculated from food and nutrient databases. There is also potential for remote dietary assessment apps to connect with health-tracking devices that can provide additional context to a patient's dietary history. 
% For example, energy expenditure can be calculated from one's smartwatch and used to verify logged intake. 

% \subsubsection{Limitations}
% Remote nutrition assessments inherit common telehealth problems, including wireless signal and camera/microphone quality issues. The accuracy of health tracking devices used to aid these assessments varies and they must be referenced consistently over time to provide meaningful information to the clinician. Remote dietary assessment methods are not immune from the limitations in dietary intake logging described previously. 
% % They still rely on self-reporting, and that error can be confounded by inaccuracies in calculated nutritional metrics from ML models or nutrient databases. 
% Even in light of these limitations, remote assessment methods can be as effective as traditional methods, while being more accessible \cite{mauldin_performing_2021}. 
% Careful consideration of the individual factors of nutrition and how they interact is just as, if not more, critical to remote assessment as it is to traditional assessment. Therefore, as telehealth becomes increasingly popular, the tools used by clinicians to collect and analyze nutritional data become increasingly important. 

==> Sections/4_x_AI_ML.tex <==
% \paragraph{Background}
We explore the potential of ML and artificial intelligence (AI) to illustrate the connections between measurable health information and micronutrient status that have eluded current clinical research. With great care and consideration, AI has a unique potential in its ability to take into account the complex personal health factors that influence diet-related health outcomes \cite{cote_artificial_2022}. 
% Machine learning is unique in its ability to find connections between different, non-linearly related features and use these connections to solve problems. Nutrition is best evaluated by a more holistic approach, taking several factors about the individual into account. 
Reviews by \citet{cote_artificial_2022} and \citet{sak_artificial_2021} outline the present state of AI for nutrition. A common approach to estimating nutritional status is by making predictions from biomarker or demographic data using ML. Such methods have been used to assess micronutrients directly \cite{truijen_predicting_2021, kurstjens_automated_2022, khan_machine_2021}. A summary of AI and ML-based methods is found in Table \ref{tab: emerging-ai}. 

% \paragraph{Developed Tools and Applications}
\subsubsection{Measuring Multiple Micronutrients Simultaneously}
Detecting multiple micronutrients in a complex sample is a critical challenge for spectroscopic methods, but computational approaches have aimed to solve this \cite{monakhova_chemometrics-assisted_2010}. Independent component analysis (ICA) is the traditional means of separating a multivariate signal into individual constituents, but ICA is often unreliable for spectra of a complex solution. Mutual Information Least Dependent Component Analysis (MILCA) was proposed as an alternative, searching for the least dependent components in a sample. The algorithm was applied to determine concentrations of vitamins C, B3, B6, A and E in various mixtures using spectra obtained with UV-visible spectrophotometry in the 200-450 nm range. In solutions made up of a combination of known concentrations of vitamin standards, MILCA outperformed other signal decomposition approaches. The authors noted that MILCA is highly sensitive to factors that impact the state of a sample such as pH, hydrolysis, and redox reactions. This evidence that individual micronutrients can be quantified in a complex mixture with a method as relatively simple as spectrophotometry is incredibly promising for future accessible methods of status assessment.

\subsubsection{Multiple Micronutrient Malnutrition Detection} \citet{truijen_predicting_2021} focused on micronutrient malnutrition in older populations, noting how malnutrition in older adults is often diagnosed too late despite the existence of screening methods. The goal of the study was to classify each sample as having either no micronutrient deficiency or 1 or more deficiencies among vitamins C, B6, B12, selenium, and zinc, confirmed by blood tests. These particular micronutrients were selected because they were not highly coordinated with each other, were among the most prevalent deficiencies, had clinically relevant cutoff points for deficiency. Logistic regression was applied to routine biochemical and diagnostic data from 9 years of United Kingdom National Diet and Nutrition Surveys (NDNS) for ages $\geq$50. Approaches such as this can suffer from ethnic disparities, with the authors noting limited generalizability to ethnic groups due to $\geq$95\% of NDNS participants being white. 

\subsubsection{Predictive Micronutrient Assessment} \citet{kurstjens_automated_2022} aimed to develop an ML algorithm to assess risk of low body iron storage (ferritin plasma levels) in anemic primary care patients using complete blood count (CBC) and CRP tests. Two algorithms were developed, each based on laboratory ferritin results from different chemistry analyzers (from Siemens and Roche). Interestingly, the two most important features were both derived from CBC test results. The authors took an important step to consider how such a model could assist a clinician by asking professionals to indicate whether a patient had low ferritin based on CBC and CRP, with and without algorithm results. Detection of low Vitamin B12 and folic acid (B9) levels were also considered, but this yielded poor results with AUCs of 0.52 and 0.57 respectively. A different study used hospital outpatient data collected over three months to predict whether a patient had normal or abnormal ferritin (iron) status \cite{luo_using_2016}. The collected data included age, sex, ferritin test results (used as targets), and other ‘predictor’ test results that were conducted in the main hospital lab only. These authors also considered the broader clinical utility of ML-powered insights, claiming that “predicted ferritin results may sometimes better reflect underlying iron status than measured ferritin” \cite{luo_using_2016}. This conclusion was based on dual independent review by pathologists on 26 selected cases where measured and predicted ferritin were `highly discrepant’. They proposed that predicted levels could be used to flag lab-measured ferritin for further review.

\input{Tables/emerging/emerging-ai}

==> Sections/4_x_Sweat.tex <==
\paragraph{Background}
% \paragraph{Measurement Approaches}  Colorimetrics uses reagents to react with sweat and change color to indicate concentrations of target substances. This color can be analyzed by a camera, such as in a smartphone as demonstrated in Figure \ref{fig:smartphone-colorimetry} by \citet{kong_accessory-free_2019}. 
% Multiplexed analyses combine and analyze data from assays with multiple sensors such as ECG, temperature, EDA, HRV data and more. Thus, these multiplexed sensors can enable more complex physiologic monitoring and diagnosis.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{Figures/Fig 1, Kong et al.png}
%     \caption{A smartphone camera and LED flash can be used to analyze results from a colorimetric assay. Used with permission from \cite{kong_accessory-free_2019}.}
%     \label{fig:smartphone-colorimetry}
%     \Description{TODO: alt text}
% \end{figure}

% \paragraph{Microfluidics} Most sweat-based sensors use microfluidic devices for the collection of sweat \cite{jo_review_2021}. These devices use very tiny valves and channels to "capture and store sweat on the surface of the subject’s skin" via the natural pressure of sweat glands \cite{jo_review_2021}. Two examples can be seen in Figures \ref{fig:microfluidics-colorimetric} and \ref{fig:microfluidics-multi}. For a more in-depth review of the nuances of creating wearable multimodal sensors with sweat collection and analysis capabilities, we direct the reader to \cite{yokus_integrated_2021}.  A summary of sweat-based methods is found in Table \ref{tab: emerging-sweat}. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{Figures/Schematic illustrations and optical images of a miniaturized sweat microfluidic device, Kim.jpg}
%     \caption{The design of a colorimetric sweat sensor using microfluidics. Used with permission from \cite{kim_skininterfaced_2022}.}
%     \label{fig:microfluidics-colorimetric}
%     \Description{TODO: alt text}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{Figures/Schematic illustrations and optical images of a skeletal microfluidic device, Kim.jpg}
%     \caption{The design of a multiplexed sweat sensor using microfluidics. Used with permission from \cite{kim_soft_2020}.}
%     \label{fig:microfluidics-multi}
%     \Description{TODO: alt text}
% \end{figure}

\paragraph{Developed Tools and Applications}
% \paragraph{Colorimetric Sensors} With our knowledge of eccrine sweat composition in mind, we look to a paper by \citet{kim_skininterfaced_2022} describing on-body colorimetric measurement of vitamin C, calcium, zinc, and iron using sweat as a biofluid (Fig. \ref{fig:microfluidics-colorimetric}). A bespoke colorimetric assay is used for each micronutrient, assessed with known concentrations in a buffer solution. Since temperature and pH can affect colorimetric results, the authors conducted tests within the normal range of body temperature and pH in sweat, finding only a slight shift in results. Uniquely, micronutrients can be supplemented transdermally through the patch itself. Multiple on-body tests were conducted. Sweat was induced by a sauna before and after supplementation (either orally or transdermally). Patch-based measurements were found to be correlated with ICP-MS results. Although the paper claims that "sweat chemistry correlates, at least semiquantitatively, to plasma chemistry" for these micronutrients \cite{kim_skininterfaced_2022}, this claim is based on the time dynamics of concentrations after supplementation rather than a comparison to a gold-standard status assessment. Furthermore, the clinical literature points out that that vitamin C and iron concentrations in sweat have been shown to have little to no correlation with levels in blood \cite{baker_physiological_2020, baker_physiology_2019}. Therefore, we argue that this device provides insights into the rate of excretion of these micronutrients rather than their status. There is also no analysis of possible measurement bias induced by transdermal supplementation at the point of sweat collection. 

% \paragraph{Electrochemical Sensors} Electrochemical analysis is pervasive in the measurement of micronutrients in sweat \cite{kim_wearable_2015,sempionatto_epidermal_2020, zhu_nonenzymatic_2023}. \citet{kim_wearable_2015} designed a square wave anodic stripping-voltammetric sensor has been used to monitor zinc in sweat during physical activity. The sensor itself is wearable, printed on tattoo transfer paper.
% % The authors thoroughly evaluated the sensor, testing its repeatability and ability to hold up against bending and stretching. 
% Assessment was conducted with standard zinc solutions in a buffer medium, covering the range of physiological concentrations of zinc in sweat. On-body experiments demonstrated the sensor's ability to detect the presence of zinc in sweat induced from cycling. A linear calibration equation was used to quantify zinc concentrations, which were found to be close to the physiological range of zinc in sweat. Again, no gold-standard assessment methods for individual zinc status were used for comparison, but this is less of a concern since this work focuses on providing insights into zinc excretion through sweat. The authors note the potential of applying this approach to other minerals found in sweat. 

% Vitamin C is targeted by \citet{sempionatto_epidermal_2020}, who deployed amperometry and immobilized ascorbate oxidase in a similar, tattoo-based form factor. Tests on human subjects focused on the temporal characteristics of the current response, finding peak response in sweat 90 minutes after supplementation and a return to baseline 180 minutes after, in line with the plasma response of vitamin C. Tears and saliva are noted as other possible biofluids, with tears yielding a similar temporal profile (albeit with different peak currents). The authors also experimented with providing different amounts of vitamin C through both supplements and orange juice, claiming the response from sweat samples to increase in line with increasing vitamin C content. Crucially, no statistical analysis was conducted on the results of the experiments, such as correlations between intake and measured current. There are also no comparisons made to clinical reference methods of vitamin C assessment, though this is stated as a subject for future work. Another flexible, electrochemical sweat biosensor for vitamin C used polyaniline film modified with phytic acid \cite{zhu_nonenzymatic_2023}. The biosensor was validated with synthesized vitamin C samples of known concentrations. Human subjects were given supplements and had their sweat collected 3 times over 90 minutes. The sensor was able to detect a general increase in current from the sweat samples over time, with variation across subjects. Saliva tests were also conducted. Peak current occurred 60 minutes after supplementation, in line with results from \cite{sempionatto_epidermal_2020}.

% \paragraph{Multiplexed Sensors} This last device is an on-body biosensing platform that can collect and analyze cortisol, glucose, and vitamin C in sweat using microfluidics \cite{kim_soft_2020} (Fig. \ref{fig:microfluidics-multi}). What makes this device a 'platform' is the integration of multiple sensing techniques: it includes a lateral flow assay for cortisol and fluorometric assays for glucose and vitamin C. Assay results are imaged with a smartphone (with special lenses in the case of fluorometry) and are analyzed to yield quantitative results. There are also electrodes for sweat rate and EDA, with NFC and RF to power them and communicate results. The focus in this paper is on stress indicators. Field-testing of the device involved subjecting participants to “intensive work periods” (interrupted sleep schedule and caffeine intake) for 7 days then rest (regular schedule) and daily vitamin C intake (for 2 participants) for 14 days \cite{kim_soft_2020}. The authors also claim they were able to assess changes in circadian rhythms through cortisol. Spikes in vitamin C associated with intake could also be observed. No trends in glucose were found. 

\input{Tables/emerging/emerging-sweat}

==> Sections/5_Precision.tex <==
Precision nutrition can be thought of as the bridge between clinical and technical methods of micronutrient assessment. It brings in the technology that can address the aforementioned limitations of clinical methods. Precision nutrition is the idea that a healthy diet changes between individuals based on how their body responds to the food they eat \cite{harvard_school_of_public_health_precision_2020}. The amount of a particular nutrient a person needs and how it is absorbed in their body can depend on their race, ethnicity, socioeconomic factors, medical history, genetics, their bacterial microbiome, and many more factors. Precision (or personalized) nutrition attempts to understand and account for all of these factors (Fig. \ref{fig:precision-nutrition-features}), and it contains methods that both directly and indirectly assess micronutrient status. Precision nutrition is a way to gather the necessary data to asses micronutrient status in a personalized manner, and when received from many people, actually has the power to inform intervention programs at a population scale. We discuss the direct and then indirect aspects, followed by limitations.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.3\linewidth]{Figures/Features of Precision Nutrition, Kirk.jpg}
  \caption{Precision nutrition has a variety of interdependent features that can be analyzed. Used with permission from \cite{kirk_precision_2021}.}
  \label{fig:precision-nutrition-features}
  \Description{Features include: Personal data, genetics, nutrigenomics, clinical and biochemical parameters, microbiome, activity tracking, meal timing, meal content, metabolomics, anthropormorphic data, and dietary intake data.}
\end{figure}

\subsection{Direct Assessments} Critical to precision nutrition is the assessment of progress resulting from nutritional interventions \cite{srinivasan_precision_2017}. This is a challenge given that conventional methods of quantitative nutritional status assessment require bulky, expensive laboratory analyzers. Emerging methods of improved portable and point of care (POC) nutrient status assessment are the enabling factors for precision nutrition. A review notes several avenues for improvement in these portable and POC devices \cite{srinivasan_precision_2017}. Mirofluidic and lab-on-chip (LoC) devices can provide real-time diagnostics and monitoring with small volumes of biological samples. They have the added benefit of being cost-effective, portable, fast, and highly sensitive. Data logging and management is another area PoC devices can improve in. To be successful, a PoC test should make results immediately available and actionable. This can be achieved through the use of smartphones or integration with lab/hospital information systems. There is also the promise of smartphone-based PoC solutions. Smartphones are ubiquitous, containing processing power, display capabilities, imaging hardware, and more. Creating a testing interface with the smartphone could unlock many new methods of status assessment. 

\subsection{Indirect Assessments} Nutrition smartphone applications are another tool that can be used to assess micronutrient status. Several works expand on the unique potential of smartphones, focusing on what makes a good nutrition app \cite{zmora_harnessing_2021}. An ideal nutrition app should “comply with a standardized Nutrition Care Process (NCP)”, “ensure efficient and reliable remote continuous care”, provide a quick and easy way to log diet, have supporting features such as dietary planning, tailor their design to a specific user base, use food databases that are current and adapted the country of the user, implement intervention decision-making based on established clinical tools, and have a strong focus on user data protection \cite{zmora_harnessing_2021} (Fig. \ref{fig:nutrition-app-reqs}). The authors also outline a hierarchy of functions for nutrition apps (Fig. \ref{fig:nutrition-app-funcs}). Apps with these features can be used to personalize diet suggestions through the data they collect with the sensors on the smartphone itself. The authors also recognize the promise of ML techniques to allow for recognition of environmental factors affecting dietary patterns and individual responses to food and intervention that can then guide suggestions. 

\begin{figure}[h]
  \centering
  \includegraphics[width=0.4\linewidth]{Figures/Requirements of nutrition apps, Zmora.png}
  \caption{Nutrition apps should meet a set of requirements associated with user input, data mining, and the app's output. Adopted with permission from Elinav and colleagues ‘Harnessing SmartPhones to Personalize Nutrition in a Time of Global Pandemic’, Nutrients 2021 \cite{zmora_harnessing_2021}. The original figure was created with a licensed version of Biorender.}
  \label{fig:nutrition-app-reqs}
  \Description{TODO: alt text}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.3\linewidth]{Figures/Strata of nutrition app functionality, Zmora.png}
  \caption{The functions of a nutrition app form a hierarchy, with meal and activity logging at the bottom and precision-based research at the top. Adopted with permission from Elinav and colleagues ‘Harnessing SmartPhones to Personalize Nutrition in a Time of Global Pandemic’, Nutrients 2021 \cite{zmora_harnessing_2021}. The original figure was created with a licensed version of Biorender.}
  \label{fig:nutrition-app-funcs}
  \Description{TODO: alt text}
\end{figure}

\subsection{Limitations}
Precision nutrition reveals several improvements in accessibility and non-invasiveness. Laboratory analyzers, which are currently the most direct method of micronutritional status assessment, are bulky and expensive to utilize. New technologies, such as PoC assessments, improve on this aspect, however they may still be largely inaccessible due to cost and complexity. The use of commodity devices such as smartphones and smart watches could decrease these limitations, thereby generating more nutritional data. ML can also be leveraged to gain insights from various data sources and sensing modalities, thereby taking into account the holistic, individualized characteristics that are critical to nutrition. A review focusing on the application of ML in precision nutrition found that ML is only applied in a few nutrition areas, with micronutrition not being one of them \cite{kirk_precision_2021}. Precision nutrition is a promising field, however it is still in its nascent stage, especially for micronutrients, and is rife with opportunity for novel, technological innovations.


% Precision nutrition has a cost-effectiveness issue. However, we see potential in the use of more ubiquitous technology, such as smartphones and smartwatches, to lower this cost. 


==> Tables/assessment_separate.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Optimal Reference Standard Methods of Assessing Micronutrient Imbalance: Water-Soluble Vitamins. Information from \cite{holler_micronutrient_2018, zhang_review_2018, mueller_aspen_2017, berger_espen_2022, national_institutes_of_health_dietary_nodate}}\label{tab: assessment-ws}
\tiny
\begin{tabulary}{\textwidth}{>{\raggedright\arraybackslash}p{0.5in}RRRRRR}\toprule
&\multicolumn{5}{c}{Detection Standard} \\\cmidrule{2-6}
Micronutrient &Method &Biomarker &Matrix &Intervals &Impact of Inflammation \\\midrule
Vitamin B1 &Erythrocyte transketolase activity coefficient assay &Increase in erythrocyte transketolase activity &Washed red blood cells &Deficient: >25\%; Insufficient: 15-25\%; Sufficient: <15\% &None on direct plasma levels \\
Vitamin B2 &Erythrocyte glutathione reductase activity coefficient assay &Increase in erythrocyte glutathione reductase activity &Washed red blood cells &Deficient: >40\%; Insufficient: 20-40\%; Sufficient: <20\% &Decrease in plasma levels (erythrocyte assays are more stable) \\
Vitamin B3 &LC-MS/MS &Niacin metabolites (NMN and 2-pyr, limited representation of stores and recent intake) &Urine &Deficient: <5.8; Insufficient: 17.5-5.8; Sufficient: >17.5 mcmol/day &Lack of evidence \\
Vitamin B5 &LC-MS/MS &Pantothenic acid (requires enzyme pretreatment) &Whole blood &Deficient: <0.22; Sufficient: 0.35-0.59 mg/L &Lack of evidence \\
Vitamin B6 &HPLC or LC-MS/MS &pyridoxal phosphate (PLP) &Plasma or serum &Sufficient: >4.94 or >7.41 $\mu$g/L plasma PLP (varies by source) &Decrease in plasma PLP, no effect on RBC concentration \\
Vitamin B7 \cite{eng_identification_2013} &LC-MS/MS for biotin; gel densitometry for MCC/PCC \cite{mall_biotin_2010} &Biotin (less sensitive); holo-MCC and holo-PCC (only reliable markers) &Urine for biotin; WBCs for MCC/PCC &
Sufficient: 4.4-31 $\mu$g/day urinary biotin, 8.2 arbitrary units holo-MCC, 9.1 arbitrary units holo-PCC &None on biomarkers \\
Vitamin B9 &LC-MS/MS &Folate &Serum for altered exposure and recent intake; Red blood cell for long term/3 month status and storage levels &Sufficient: >3 ng/mL serum, >140 ng/mL RBC &Lack of evidence \\
Vitamin B12 \cite{adas_medical_knowledge_team_vitamin_2023}&GC-MS &B12, confirmed with methylmalonic acid (MMA, also related to B2, B6, folate); no single 'optimal reference standard' &Plasma or serum &Deficient: <200-250 pg/mL B12, >0.03 mg/L MMA (some debate over this) &Association with increased B12 levels \\
Vitamin C &HPLC &Ascorbate &Plasma (some claim serum should be avoided) &Deficient: 1.94; Insufficient: 2.11-4.05; Sufficient: 4.05 mg/L &Decrease in plasma ascorbic acid (rapid, decrease when CRP >10 mg/L, normal values not detected if CRP >40 mg/L) \\
\bottomrule
\label{tab:assess-vitamins-water-soluble}
\end{tabulary}
\end{table}

%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Optimal Reference Standard Methods of Assessing Micronutrient Imbalance: Fat-Soluble Vitamins. Information from \cite{holler_micronutrient_2018, zhang_review_2018, mueller_aspen_2017, berger_espen_2022, national_institutes_of_health_dietary_nodate}}\label{tab: assessment-fs}
\tiny
\begin{tabulary}{\textwidth}{>{\raggedright\arraybackslash}p{0.5in}RR>{\raggedleft\arraybackslash}p{0.1in}RRR}\toprule
&\multicolumn{5}{c}{Detection Standard} \\\cmidrule{2-6}
Micronutrient &Method &Biomarker &Matrix &Intervals &Impact of Inflammation \\\midrule
Vitamin A &LC-MS/MS &Retinol (only sensitive to deficiency or excess in storage, affected by infection and protein/zinc deficiency). Best method is to indirectly measure reserves in liver over several days of administration &Plasma or serum &Severely deficient: <0.1; Deficient: 0.1-0.2; Sufficient: 0.3-1; Toxic: >1 mg/L retinol &Decrease in serum retinol (adjustment equations exist but are not universally applicable, BRINDA R package) \\
Vitamin D \cite{ross_dietary_2011}&LC-MS/MS &25(OH)D (calcidiol) &Plasma or serum &Deficient: <12; Insufficient: 12-<20; Sufficient: 20-50; Toxic: >50 ng/mL (not definitively established/linked to clinical outcomes, varies based on assay and lab) &Decrease in plasma levels (all values below reference ranges with CBP >40 mg/L) \\
Vitamin E &LC-UV &Ratio of Vit E to total blood lipids &Plasma or serum &Insufficient: <5.17 mg/L Vit E, <0.8 mg Vit E/g total lipid; Sufficient: 8.6-13 mg/L Vit E (adults have higher levels) &Some effects (blood concentrations less interpretable at CRP >80 mg/L) \\
Vitamin K &Immuno-based assays &Plasma phylloquinone (usually for short term intake, no single 'optimal reference standard'); prothrombin time (time to blood clot, only clinically relevant measure); variety of other 'functional' biomarkers &Plasma &Deficient: <0.15; Sufficient (fasting): 0.15-1 $\mu$g/L &Status associated with lower inflammatory marker concentration  \\
\bottomrule
\label{tab:assess-vitamins-fat-soluble}
\end{tabulary}
\end{table}

%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Optimal Reference Standard Methods of Assessing Micronutrient Imbalance: Minerals. Information from \cite{holler_micronutrient_2018, zhang_review_2018, mueller_aspen_2017, berger_espen_2022, national_institutes_of_health_dietary_nodate}}\label{tab: assessment-min}
\tiny
\begin{tabulary}{\textwidth}{>{\raggedright\arraybackslash}p{0.5in}RRRRRR}\toprule
&\multicolumn{5}{c}{Detection Standard} \\\cmidrule{2-6}
Micronutrient &Method &Biomarker &Matrix &Intervals &Impact of Inflammation \\\midrule
Iron \cite{gloria_iron_nodate,gerber_iron_2024}&Electrochemiluminescence immunoassay (ECLIA) &Ferritin for deficiency (first phase, evaluates storage, inflated by infection); Iron increase after supplementation for malabsorption; Hemoglobin used to confirm IDA &Serum &Iron-deficiency anemia: <10, Deficiency: 10-30 $\mu$g/L ferritin &Ferritin may be inflated, falsely normal/misleading (adjustment equations exist but are not universally applicable, BRINDA R package) \\
Copper &ICP-MS &Copper or ceruloplasmin (CP), neither reliable &Serum &Depletion: <50.8 (copper); Deficient: 50.8-76.2 (copper, high CRP); Sufficient: 63.5-158.9 $\mu$g/dL (copper), 180-400 mg/L (CP) &Increase in plasma concentrations \\
Zinc \cite{pat_bass_symptoms_2023}&Atomic Absorption Spectroscopy (AAS) &Zinc (levels are halved by Systemic Inflammatory Response Syndrome, can be normal with clinical symptoms present, levels vary with time of day so it is recommended that albumin and CRP changes are taken into account) &Plasma or serum &Deficient: 70 women, 74 men; Insufficient: 70/74-80; Sufficient: 80-120 $\mu$g/dL &Decrease in plasma levels (significant when CRP exceeds 20 mg/L, adjustment equations exist but are not universally applicable, BRINDA R package)  \\
Iodine &ICP-MS &Iodine &Urine (24h or random), serum less recommended &Depletion: <20, NA; Deficient: 20-100, <40; Sufficient: 100-300 $\mu$g/24hr urine, 40-100 $\mu$g/L serum (levels should be higher in those who are pregnant or lactating) &Lack of evidence  \\
Selenium &AAS, ICP-MS &Selenium (recent intake) or Selenoprotein P &Plasma or serum &Deficient: <60; Sufficient: >60; Toxicity: >474 to 948 $\mu$g/L Se (intervals vary by source and population: women and black people have naturally lower concentrations) &Decrease in plasma levels proportional to inflammation, can be adjusted for  \\
Magnesium &AAS &Magnesium &Serum (little correlation with overall status or tissue stores) and urine (after supplementation) &Deficient: <18.23; Sufficient: 18.23-23.1 mg/L serum Mg & \\
\bottomrule
\label{tab:assess-minerals}
\end{tabulary}
\end{table}

==> Tables/emerging/emerging-assay.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Assay-Based Methods Using Sweat}\label{tab: emerging-assay-sweat}
\scriptsize
\begin{tabular}{p{0.5in}p{0.6in}p{0.4in}p{0.5in}p{0.5in}p{0.6in}p{0.75in}p{0.6in}p{0.25in}}\toprule
% \multicolumn{9}{c} {Assay-Based Methods} \\
Method &Platform&Targets &Analytes &Evaluation &Control &Results &Notes &Source
\\\midrule
% Sweat-based colorimetric sensors
Fluorometry &Wearable patch &Chloride, sodium, and zinc &Sweat &Induced sweat &Ion chromatography (chloride), AAS (sodium), ICP-MS (zinc) &Zinc measurement was the most inaccurate and subject to the most variance &Statistical analysis of results is not presented &\cite{sekine_fluorometric_2018} \\
Colorimetry &Wearable &Vitamin C, calcium, zinc, and iron &Sweat &Human subjects &ICP-MS on diluted sweat samples and supplementation &Correlations with ICP-MS of 0.926 for Vit C, 0.743 for calcium, 0.895 for zinc, and 0.963 for iron, time dynamics of measurements after supplementation were in line with those of blood &Sensor can also supplement micronutrients transdermally &\cite{kim_skininterfaced_2022} \\
% Sweat-based multiplexed sensors
Fluorometric and lateral flow assays &Wearable with smartphone analysis &Cortisol, glucose, and vitamin C &Sweat &Human subjects &ELISA for cortisol, controlled stress and diet &Cortisol aligned with circadian rhythm changes and had $R^2$ of 0.7974 with ELISA, observed spikes in Vit C with intake, no trends in glucose &Measurement of sweat rate and EDA, with NFC and RF to power them and communicate results &\cite{kim_soft_2020} \\
\bottomrule
\end{tabular}
\end{table}

% Smartphone-based
\begin{table}[!htp]\centering
\caption{Assay-Based Methods Using Smartphones}\label{tab: emerging-assay-smartphone}
\scriptsize
\begin{tabular}{p{0.5in}p{0.6in}p{0.4in}p{0.5in}p{0.5in}p{0.6in}p{0.75in}p{0.6in}p{0.25in}}\toprule
% \multicolumn{9}{c} {Assay-Based Methods} \\
Method &Platform&Targets &Analytes &Evaluation &Control &Results &Notes &Source
\\\midrule
Quantitative immunoassay &Smartphone-based &Calcidiol &Serum &Known sample solutions and serum &ELISA &Errors “at same order” as ELISA &&\cite{lee_smartphone_2014} \\
Quantitative immunoassay &Smartphone-based &Vitamin B12 &Finger prick blood sample &Human Subjects &Immulite 2000 Immunoassay &Correlation of 0.93 with control, ~85\% specificity and ~60\% sensitivity for deficiency detection &&\cite{lee_nutriphone_2016} \\
Quantitative immunoassay &Smartphone-based or portable device (TIDBIT) &Ferritin &Finger prick blood sample &Human Subjects &Immulite 2000 Immunoassay &Correlation of 0.92 with control, sensitivity of 0.9 for deficiency detection &&\cite{srinivasan_ironphone_2018} \\
Quantitative immunoassay &Smartphone-based &Iron (total) &Finger prick serum blood sample &Human Subjects &Multi-Well Plate Spectrophotometry &$R^2$ of 0.98 with control, CoV of 10.5\% &Conducted specificity testing using interferent analytes, considered toxicity &\cite{serhan_total_2020} \\
Quantitative immunoassay &Smartphone-based &Iron (total) &Finger prick whole blood sample &Human Subjects &Laboratory developed test: spectrophotometry-based technique & Calibration slope of 0.0004 au $\mu$g$^{-1}$ dL$^{-1}$, a correlation plot with slope of 1.09, R$^2$ of 0.96, and a mean bias of 5.3\%& Manually diluted some samples to represent a low iron concentration &\cite{serhan_2021} \\
Colorimetric assay &Paper-based &Iron (total) &Urine &Human subjects &AAS &RSD of 9.5\% &Urine citric acid was found to interfere with results &\cite{ferreira_new_2021} \\
Colorimetric assay &Paper-based &Iron (Fe3+) &Serum &Spiked, diluted serum &Spiked known concentration &Error of 3.7\% and RSD of 1\% &LoD of 0.3 mcg/mLl &\cite{dortez_integrated_2023} \\
Colorimetric assay &Paper-based & Iron (Fe3+) &Saliva &Spiked pooled commercial saliva &Spiked known concentration &$R^2$ of 0.99 &Ferritin is the gold-standard indicator of iron deficiency; it is debated whether salivary iron reflects circulating status &\cite{prakobdi_non-invasive_2024} \\
Opto-electronic immunoassay &Card &Ferritin, RBP, and CRP &Whole blood &Human subjects &ELISA &CVs of 2.5\% for ferritin, 10.8\% for RBP, and 3.9\% for CRP & RBP is not the clinically-accepted biomarker for Vitamin A status; Device transmits results to a smartphone over NFC &\cite{lee_flexible_2016} \\
Multiplexed quantitative assay &Portable device &RBP, Ferritin, and CRP &Serum &Serum samples &ELISA &$R^2$ of 0.56 for RBP, 0.92 for ferritin, 0.88 for CRP & RMSE for RBP was 21 mcg/mL &\cite{lu_rapid_2017} \\
Quantitative immunoassay &Portable device (TIDBIT) &Serum and whole blood &25(OH)D3 &Human subjects &LC-MS/MS & $R^2$ of 0.91 for serum tests, 0.94 for finger prick tests & &\cite{vemulapati_quantitative_2017} \\
\bottomrule
\end{tabular}
\end{table}

% Commercial
\begin{table}[!htp]\centering
\caption{Commercial Assay-Based Methods}\label{tab: emerging-assay-commercial}
\scriptsize
\begin{tabular}{p{0.5in}p{0.6in}p{0.4in}p{0.5in}p{0.5in}p{0.6in}p{0.75in}p{0.6in}p{0.25in}}\toprule
% \multicolumn{9}{c} {Assay-Based Methods} \\
Method &Platform&Targets &Analytes &Evaluation &Control &Results &Notes &Source
\\\midrule
Fluorometry &Portable device &Retinol and retinyl esters &Human milk &Human subjects &HPLC &Weak correlation ($R^2$=0.59, p<0.001), but mean difference was “not statistically different from zero” &Of major concern was the ability for the human milk to satisfy the vitamin A requirements of children &\cite{abebe_low_2019} \\
Quantitative immunoassay &Portable device &Ferritin, other tests &Finger prick blood sample &Not published &Not published &Not published &Commercially available &\cite{bloom_diagnostics_overview_2021}\\
Immunofluorescence &Portable device &Cholecalciferol &Serum &Human subjects &Abbott Alinity i immunoassay & $R^2$ of 0.89; SE of 0.16 at 10 ng/mL, 0.19 at 12 ng/mL, and 0.35 at 30 ng/mL & Standard error lower than control; recommends additional testing for excess status; target is not the clinically-accepted biomarker for Vitamin D &\cite{albrecht_rapid_2021} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/emerging/emerging-assay/smartphone_grouped.tex <==
% Smartphone-based
\begin{table}[!htp]\centering
\caption{Assay-Based Methods Using Smartphones}\label{tab: emerging-assay-smartphone}
\tiny
\begin{tabular}{p{0.5in}p{0.6in}p{0.4in}p{0.5in}p{0.5in}p{0.6in}p{0.75in}p{0.6in}p{0.25in}}\toprule
% \multicolumn{9}{c} {Assay-Based Methods} \\
Method &Platform&Targets &Analytes &Evaluation &Control &Results &Notes &Source
\\\midrule
\multirow{15}{0.5in}{Quantitative immunoassay} &\multirow{10}{0.6in}{Smartphone-based} &Vitamin D (calcidiol)&Serum &Known sample solutions and human subjects &ELISA &Errors “at same order” as ELISA & No statistical analysis of results &\cite{lee_smartphone_2014} \\
&&Vitamin B12 (cyanocobalamin) &Capillary blood sample &Human Subjects &Immulite 2000 Immunoassay &Correlation of 0.93 with control, ~85\% specificity and ~60\% sensitivity for deficiency detection &Used synthetic form of B12; poor accuracy outside of deficiency range &\cite{lee_nutriphone_2016} \\
&&Iron (total) &Capillary serum sample &Human Subjects &Multi-Well Plate Spectrophotometry &$R^2$ of 0.98 with control, CoV of 10.5\% &Conducted specificity testing using interferent analytes; considered toxicity &\cite{serhan_total_2020} \\
&&Iron (total) &Capillary blood sample &Human Subjects &Laboratory developed test: spectrophotometry-based technique & Correlation plot with slope of 1.09, R$^2$ of 0.96, and a mean bias of 5.3\%& Improved on control LoD; manually diluted some samples to represent a low iron concentration &\cite{serhan_2021} \\
\cmidrule{2-9}
&Smartphone-based or portable device (TIDBIT) &Iron (ferritin)&Capillary blood sample &Human Subjects &Immulite 2000 Immunoassay &Correlation of 0.92 with control, sensitivity of 0.9 for deficiency detection & &\cite{srinivasan_ironphone_2018} \\
&Portable device (TIDBIT) &Vitamin D3 (calcidiol) &Serum and whole blood&Commercial standards; human subjects&Known solutions; LC-MS/MS& CoV with standards of 2.63\% at 34 ng/mL and 11.2\% at 0 ng/mL; $R^2$ of 0.91 for serum tests, 0.94 for capillary blood tests&&\cite{vemulapati_quantitative_2017} \\
\cmidrule{1-9}
Colorimetric assay &Paper-based &Iron (total) &Urine &Human subjects &AAS &RSD of 9.5\% &Urine citric acid was found to interfere with results &\cite{ferreira_new_2021} \\
Colorimetric assay &Paper-based &Iron (Fe3+) &Serum &Spiked, diluted from human subjects &Spiked known concentration &Error of 3.7\% and RSD of 1\% &LoD of 0.3 $\mu$g/mLl &\cite{dortez_integrated_2023} \\
Colorimetric assay &Paper-based & Iron (Fe3+) &Saliva &Spiked pooled commercial saliva &Spiked known concentration &$R^2$ of 0.99 &It is debated whether salivary iron reflects circulating status &\cite{prakobdi_non-invasive_2024} \\
Opto-electronic immunoassay &Card &Vitamin A (RBP), Iron (ferritin), and CRP &Whole blood &Human subjects &ELISA &CVs of 2.5\% for ferritin, 10.8\% for RBP, and 3.9\% for CRP &Cutoff for iron deficiency was insensitive to upper limit; RBP is not the clinically-accepted biomarker for vitamin A status; Device transmits results to a smartphone over NFC &\cite{lee_flexible_2016} \\
Multiplexed quantitative assay &Portable device (TIDBIT) &Vitamin A (RBP), Iron (ferritin), and CRP &Serum &Human subjects &ELISA &$R^2$ of 0.56 for RBP, 0.92 for ferritin, 0.88 for CRP &Ferritin range does not cover anemia; RBP is not the clinically-accepted biomarker for vitamin A status; RMSE for RBP was 21 $\mu$g/mL &\cite{lu_rapid_2017} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/emerging/emerging-electro.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Electrochemical Methods}\label{tab: emerging-electro}
\scriptsize
\begin{tabular}{p{0.55in}p{0.5in}p{0.45in}p{0.5in}p{0.5in}p{0.6in}p{0.7in}p{0.7in}p{0.2in}}\toprule
% \multicolumn{9}{c}{Electrochemical Methods} \\
% \cmidrule{1-9}
Method &Platform&Targets &Analytes &Evaluation &Control &Results &Notes &Source
\\\midrule
% Voltammetry
Voltammetry &Benchtop &Vitamins B2 (riboflavin), B9 (folic acid), and C (ascorbic acid) &Plasma &Human subjects &Spiked known concentrations &>99\% recovery of spiked concentrations &Tested in 7.2 pH buffer, which is slightly higher than pH of blood ($\sim$7.4); direct riboflavin is not the gold-standard biomarker for Vitamin B2; folic acid is the synthetic form of folate; Linear range for vitamin C is 1000x physiological intervals &\cite{revin_simultaneous_2012} \\
Anodic stripping voltammetry &Benchtop &Zinc &Serum &Human subjects &Spiked known concentrations &Peak current decreased with concentration, but were lower in magnitude than buffer &A sample pH of 6 was necessary for optimal performance &\cite{jothimuthu_zinc_2013} \\
Square wave voltammetry &Benchtop &Vitamin B9 (folic acid), GSH, and NADH &Urine and serum &Human subjects (urine only) &Spiked with known concentrations &Accurate recovery of spiked concentration & Simultaneous determination of targets; unclear whether pre-existing urine composition biased recovery; claims serum evaluation but this is not presented; folic acid is the synthetic form of folate &\cite{raoof_high_2015} \\
Square wave anodic stripping-voltammetry &Wearable tattoo&Zinc &Sweat &Zinc stock solutions &Known zinc solutions &$R^2$ of 0.999 for measured current vs stock solutions, LoD of 0.05 mcg/mL &Zinc content in actual sweat from single participant was close to physiological range &\cite{kim_wearable_2015} \\
Square wave anodic stripping voltammetry &Wearable patch &Zn, Cd, Pb, Cu, and Hg ions &Sweat and urine &Human subjects &ICP-MS &Similar to control, but provided no statistical analysis &Included temperature sensor to account for the influence of skin temperature on peak current &\cite{gao_wearable_2016} \\
Square wave voltammetry &Benchtop &Vitamin B12 (cyanocobalamin) &Urine &Diluted from human subjects &Spiked with known concentrations &98-105\% recovery &Cyanocobalamin is the synthetic form of B12 &\cite{stankovic_electroanalytical_2016} \\
Square wave voltammetry and chronoamperometry &Eyeglasses&Vitamins B2, B6, and C, alcohol, and glucose &Induced tears &Human subjects &Breathalyzer BAC, commercial glucometer, vitamin supplementation &Correlations of 0.852 with BAC, ~0.7 with glucometer, distinct voltage peaks for each vitamin &Glucose and alcohol was main focus, vitamin assessment included as a proof of concept; exact form of each vitamin is not known &\cite{sempionatto_eyeglasses-based_2019} \\
Cyclic voltammetry &Benchtop &Iron (ferritin) &Serum &Spiked from human subjects &ELISA &$R^2$ of 0.966 and lower linearity than control &Studied the impact of pH and interferent compounds &\cite{garg_microfluidic-based_2020} \\
Cyclic voltammetry &Nanodevice with handheld analyzer &Vitamin C &Serum &Human subjects &HPLC & $R^2$ of 0.984 (p<0.001) and 100\% accuracy in deficiency detection &Targets scurvy (extreme deficiency) &\cite{sun_bendable_2021} \\
Voltammetry &Wearable patch &Vitamins B6, C, D3, E, and other macronutrients and amino acids &Sweat &Not reported for vitamins &Not reported for vitamins &Observable linear relationship between vitamin concentration and peak height current density &Quantitative results for vitamins were not reported &\cite{wang_wearable_2022} \\
Voltammetry & Benchtop instrument & Vitamin D3 & Plasma & Spiked from human subjects & Spiked known concentrations and HPLC-UV & LoD of 1.9 ng/mL; RSD of 0.3-2.6\% and recovery of 96-102\% &Exact form of D3 (gold-standard 25(OH)D3/calcidiol or calciol) not reported &\cite{kumar2023} \\
Square wave voltammetry and potentiometric measurement & Portable sensor & Zinc and vitamin C (ascorbic acid) & Fingertip sweat & Human subjects & Supplementation & Both micros could be analyzed over time simultaneously & No comparison to clinical assessment of status or statistical analysis of results; Vitamin C range far exceeded physiological concentrations in plasma & \cite{Seker2024} \\
Differential pulse voltammetry &Wearable patch &Vitamin B2 (riboflavin) &Sweat &Human subjects &HPLC &$R^2$ of 0.9783 with sweat HPLC and 0.87 with urine fluorescence spectroscopy &Urine included as comparison to sweat status; incorporates pH sensor to control for influence of pH on measurements; direct riboflavin is not the gold-standard biomarker for Vitamin B2 status &\cite{shi_wireless_2024} \\

% Amperometry
Amperometry &Benchtop &Vitamin B9 (folic acid) &Serum &Human subjects &Spiked known concentrations &>99\% recovery of spiked concentration &Robust against interference from ascorbic acid; sensor performance peaked at pH 7.2, slightly lower than pH of serum; folic acid is the synthetic form of folate &\cite{maiyalagan_nanostructured_2013} \\
Amperometry &Wearable tattoo&Vitamin C &Sweat, tears, and saliva &Human subjects &Supplementation &Similar time dynamics to plasma for tears and sweat & &\cite{sempionatto_epidermal_2020} \\
Amperometry&Wearable sensor chip&Vitamin C &Sweat, urine, and blood &Human subjects &Supplementation/ intake, blood measurements with the same sensor &Urine and sweat measurements increased after intake, with inter-trial variation. Correlations with blood sensor measurements were 0.81 for sweat and 0.72 for urine &Used emergen-C as a vitamin C supplement, which contains several other micronutrients &\cite{zhao_wearable_2021} \\
Electrocatalytic vitamin C amperometric assay and competitive vitamin D immunoassay &Point of care&Vitamins C and D (calcidiol) &Saliva &Human subjects &Vitamin supplementation &Observable rise and drop in levels over time &Saliva sample must be pre-treated, Vitamin C has little assessment &\cite{ruiz-valdepenas_montiel_decentralized_2021} \\
% Amperometry with a graphene-based field effect transistor&Point of care&Ferritin &Electrolyte buffer solution &Ferritin stock solutions &Known ferritin concentrations &Resistance measurements decreased with increasing ferritin concentrations, detection range of 5.3 ng/L to 0.5 mcg/L &Goal was to non-invasively detect iron deficiency in children through saliva samples &\cite{oshin_graphene-based_2020} \\
Amperometry&Wearable sensor chip &Vitamin C &Sweat and saliva &Stock solutions and human subjects &Known solutions and supplementation &$R^2$ of 0.99 and LoD of 0.0299 mcg/mL for stock solutions, was able to detect general increase in current after supplementation & &\cite{zhu_nonenzymatic_2023} \\
Chronoamperometry & Wearable sensing system & Vitamin C (ascorbic acid) and Levodopa & Sweat & Human subjects & Vitamin supplementation &
% The sensitivities of the levodopa sensor and the vitamin C sensor are 0.0073 and 0.0018 $\mu$A$\cdot$$\mu$M$^{-1}$, respectively, and the 
Detection correlation coefficients of both exceed 0.99; both sensors have a wide linear detection range of 0-17.6 mg/L and 0-1000 $\mu$M, respectively, and low detection limits of 0.05 mg/L and 17.9 $\mu$M, respectively. & The system is wireless, battery-free, flexible, finger-actuated, and self-pumping \cite{Ning2024} \\

% Other
Arm impedance measurement scan &Non-mobile, clinical device &Vitamin D &Impedance measurement at 21.1 Hz &Human subjects &Vitamin D status by blood test (method unspecified) &$R^2$ of 0.75 (regression with Vitamin D level) &Also evaluated regression models with medical checkup and body composition analysis data &\cite{heo_novel_2021} \\
Electroacupuncture &Point of care&26 different vitamins and minerals &Electrical resistance on the surface of the skin &Not published &Not published &Not published &Should only be used as an indicator of "general vitamin trend" &\cite{noauthor_support_2023} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/emerging/emerging-image.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Emerging Image-Based Methods}\label{tab: emerging-image}
\scriptsize
\begin{tabular}{p{0.5in}p{0.5in}p{0.5in}p{0.5in}p{0.5in}p{0.6in}p{0.75in}p{0.6in}p{0.25in}}\toprule
\multicolumn{9}{c}{Image-Based Methods} \\\cmidrule{1-9}
Method &Platform&Targets &Analytes &Evaluation &Control &Results &Notes &Source
\\\midrule
FFT and SVM &Smartphone &Hemoglobin, Anemia &Fingertip &Human subjects &Blood Hemoglobin (Masimo Pronto optical device) &0.82 rank order correlation for anemia classification &Used 880 and 970 nm light sources &\cite{wang_hemaapp_2016} \\
ANN &Smartphone &Hemoglobin &Fingertip &Human subjects &Blood Hemoglobin &0.93 rank of correlation &Took age and gender into consideration, able to identify regions with high variance &\cite{hasan_smarthelp_2018} \\
Image Analysis and Stepwise Regression &Smartphone &Hemoglobin, Anemia &Conjunctiva &Human subjects &Blood Hemoglobin (pulse oximeter) &AUC of 0.8 for anemia prediction &Robust considerations for skin color &\cite{suner_prediction_2021} \\
Linear Regression &Handheld camera &TC and LDL &Corneal Lipid Deposition &Human subjects &Blood TC and LDL &Correlations of 0.986, 0.968, 0.974, and 0.932 for 40-60 TC, 40-60 LDL, >60 TC, and >60 LDL, respectively &Targeted age groups of 40-60 and >60 &\cite{kumar_non-invasive_2016} \\
Linear Regression &Handheld &TC &Fingertip &Human subjects &Blood TC &$R^2$ of 0.9747 &Used 940 nm light source &\cite{umar_real_2020} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/emerging/emerging-sweat.tex <==
%Please add the following packages if necessary:
% \usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Sweat-Based Methods}\label{tab: emerging-sweat}
\scriptsize
\begin{tabular}{p{0.5in}p{0.4in}p{0.45in}p{0.4in}p{0.55in}p{0.55in}p{0.95in}p{0.65in}p{0.25in}}\toprule
\multicolumn{9}{c}{Sweat-Based Methods} \\\cmidrule{1-9}
Method &Platform&Targets &Analytes &Evaluation &Control &Results &Notes &Source
\\\midrule
Square wave anodic stripping-voltammetry &Tattoo &Zinc &Sweat &Zinc stock solutions &Known zinc solutions &$R^2$ of 0.999 for measured current vs stock solutions, LoD of 0.05 mcg/mL &Zinc content in actual sweat from single participant was close to physiological range &\cite{kim_wearable_2015} \\
Colorimetry &Wearable &Vitamin C, calcium, zinc, and iron &Sweat &Human subjects &ICP-MS on diluted sweat samples and supplementation &Correlations with ICP-MS of 0.926 for Vit C, 0.743 for calcium, 0.895 for zinc, and 0.963 for iron, time dynamics of measurements after supplementation were in line with those of blood &Sensor can also supplement micronutrients transdermally &\cite{kim_skininterfaced_2022} \\
Amperometry &Tattoo &Vitamin C &Sweat, tears, and saliva &Human subjects &Supplementation &Similar time dynamics to plasma for tears and sweat & &\cite{sempionatto_epidermal_2020} \\
Electrochemistry &Sensor chip &Vitamin C &Sweat and saliva &Stock solutions and human subjects &Known solutions and supplementation &$R^2$ of 0.99 and LoD of 0.0299 mcg/mL for stock solutions, was able to detect general increase in current after supplementation & &\cite{zhu_nonenzymatic_2023} \\
Fluorometry and lateral flow assays &Wearable with smartphone analysis &Cortisol, glucose, and vitamin C &Sweat &Human subjects &ELISA for cortisol, controlled stress and diet &Cortisol aligned with circadian rhythm changes and had $R^2$ of 0.7974 with ELISA, observed spikes in Vit C with intake, no trends in glucose &Measurement of sweat rate and EDA, with NFC and RF to power them and communicate results &\cite{kim_soft_2020} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/test_cost.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage{xcolor,colortbl} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Estimated Cost of Optimal Reference Standard Laboratory Testing}\label{tab: cost}
\scriptsize
\begin{tabular}{lrrrr}\toprule
Laboratory Test &Relevant Micronutrients &Estimated Cost &Provider \\\midrule
LC-MS &B3, B5, B6, B7, B9, A, D &\$57.16 / analysis &Harvard Center for Mass Spectrometry \\
HPLC-Vis &Pro-vitamin A carotenoids &No Estimate Available & \\
LC-UV &E &No Estimate Available & \\
Immuno-based Assays &K &\$13.75 / result &Bio-Techne \\
ECLIA &Fe &\$59 / test &Quest Diagnostics \\
Nephelometry,Turbidimetry &Cu &\$44 / test &Walk-In Lab \\
AAS &Zn &\$149.85 / element &MSE Supplies \\
ICP-MS Immunoassay &Se, Mn &\$80.95 / element &MSE Supplies \\
Photometric &I &\$75.65 / test &Walk-In Lab \\
ETKac Assay &B1 &\$65 / test &Walk-In Lab \\
EGRac Assay &B2 &\$120 / test &Walk-In Lab \\
GC-MS &B12 &\$137.19 / analysis &Harvard Center for Mass Spectrometry \\
HPLC &C &No Estimate Available & \\
\bottomrule
\end{tabular}
\end{table}
